Towards urban scenes understanding through polarization cues

Autonomous robotics is critically affected by the robustness of its scene understanding algorithms. We propose a two-axis pipeline based on polarization indices to analyze dynamic urban scenes. As robots evolve in unknown environments, they are prone to encountering specular obstacles. Usually, specular phenomena are rarely taken into account by algorithms which causes misinterpretations and erroneous estimates. By exploiting all the light properties, systems can greatly increase their robustness to events. In addition to the conventional photometric characteristics, we propose to include polarization sensing. We demonstrate in this paper that the contribution of polarization measurement increases both the performances of segmentation and the quality of depth estimation. Our polarimetry-based approaches are compared here with other state-of-the-art RGB-centric methods showing interest of using polarization imaging.

==> Autonomous Robots_arxiv_fin/biographies.tex <==


  \begin{wrapfigure}{l}{25mm} 
    \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author-fig1.jpg}
  \end{wrapfigure}
  \textbf{Marc Blanchon} is a third-year Ph.D Student in Universit\'e Bourgogne Franche-Comt\'e in the EMR VIBOT CNRS 6000 team. He recieved a Bachelor's degree and a Master's degree both in Computer Vision from Universit\'e Bourgogne Franche-Comt\'e in 2016 and 2018 respectively. His main research interests are computer vision for autonomous  vehicles and physics-based deep learning. \vspace{.1cm}\\
  
  \begin{wrapfigure}{l}{25mm} 
    \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author-fig2.jpg}
  \end{wrapfigure}
  \textbf{D\'esir\'e Sidib\'e} received a Master degree from Ecole Centrale de Nantes and a Ph.D from Universit\'e de Montpellier in 2004 and 2007 respectively. From 2009 to 2019, he was an assistant, then associate professor at Universit\'e de Bourgogne and a member of the Le2i laboratory. Since 2019, he is a professor at Universit\'e Paris Saclay and a member of the IBISC laboratory. His main research areas include computer vision for autonomous vehicles, and medical image analysis. He has authored and co-authored more than 80 papers in international journals and conferences. He is a senior member of IEEE.\vspace{.1cm}\\
  
    \begin{wrapfigure}{l}{25mm} 
    \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author-fig3.jpg}
  \end{wrapfigure}
  \textbf{Olivier Morel} received his MSc degree in computer vision and image processing from the University of Burgundy in 2002. In November 2005, he received his PhD degree in computer vision from the University of Burgundy. Since September 2007, he has worked as a lecturer in the VIBOT Team EMR CNRS 6000 from University of Bourgogne Franche-Comt\'e. His main research interests are polarization imaging and the applications of polarimetric vision to robotics and unmanned vehicles.\vspace{.1cm}\vfill
  
    \begin{wrapfigure}{l}{25mm} 
    \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author-fig4.jpg}
  \end{wrapfigure}
  \textbf{Ralph Seulin} is a research engineer at CNRS in EMR VIBOT CNRS 6000 team. In 2002, he received his Ph.D degree in computer vision from the University of Burgundy. His main research areas include robotics, and computer vision for autonomous vehicles.
  He has authored and co-authored more than 80 international publications.\vspace{.1cm}\\
  
    \begin{wrapfigure}{l}{25mm} 
    \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author-fig5.png}
  \end{wrapfigure}
  \textbf{Fabrice Meriaudeau} received both the master degree in physics at Dijon University, France as well as an Engineering Degree (FIRST) in material sciences in 1994. He also obtained a Ph.D. in image processing at the same University in 1997. He was a postdoc for a year at The Oak Ridge National Laboratory. He is currently Professeur des Universit\'es at the University of Burgundy.
He was the director of the Institute Health and Analytics (2017/2018) at the Universiti Teknologi PETRONAS Malaysia and was the Director of the Le2i (UMR CNRS) France, which has more than 200 staff members, from 2011 to 2016. His research interests were focused on image processing for non-conventional imaging systems (UV, IR, polarization) and more recently on medical/biomedical imaging. He coordinated an Erasmus Mundus Master in the field of Computer Vision and Robotics from 2006 to 2010 and was the Vice President for International Affairs for the University of Burgundy from 2010 to 2012. He has authored and co-authored more than 150 international publications and holds three patents.

==> Autonomous Robots_arxiv_fin/differentiation.tex <==
\colorlet{crystal}{gray}
	
	\def\zangle{-20}
	\def\xangle{20}
	
	\begin{tikzpicture}[x=(\xangle:0.75cm), y=(90:1cm), z=(\zangle:1.5cm),
	>=stealth, line cap=round, line join=round,
	lines/.style={gray!70, thick}, 
	axis/.style={black, thick},
	plate/.style={fill, opacity=0.875},
	markers/.style={darkgray!80, thick},
	markerss/.style={black!30, thick}]
	
	
	
	
	\begin{scope}[shift={(0,0,3.125)}]
	
	\node [yslant=tan(\zangle), above=0.25cm, align=center,font=\footnotesize] at 
	(1,1,1.5){Linearly Polarized Light};
	
	\begin{scope}[xscale=1.5, yscale=1.5]
	\path [crystal!25, plate] 
	(-1,-1,0) -- (-1,1,0) -- (1,1,0) -- (1,-1,0) -- cycle;
	\path [crystal!50, plate] 
	(-1,-1,0) -- (-1,-1,-0.125) -- (-1,1,-0.125) -- (-1,1, 0) -- cycle;
	\path [crystal!75, plate] 
	(-1,1,0) -- (-1,1,-0.125) -- (1,1,-0.125) -- (1,1, 0) -- cycle;
	\node [yslant=tan(\xangle), text=crystal!50, below, font=\small] at 
	(-1.125,-1,0){Sensor};
	\end{scope}
	
	
	\draw [markers] (0,1) -- (0,-1) (-0.5,0) -- (0.5,0);
	
	\draw [axis] (0,0,0) -- (0,0,3);
	
	\foreach \k [evaluate={%
		\i=\k*5.625; \j=\i>0 ? \i-5.625 : 0; 
		\a=90-\i; 
		\b=90-\j; 
		\c=int(mod(\k,4)==0 && sin \a != 0); 
		\d=int(\k+1/4);}] in {0,...,192}{
		\ifodd\d
		\ifnum\c=1
		\draw [->,opacity=0.3] (0,0,\i/360) -- ++(sin \a, sin \a, 0);
		\fi
		\draw [thick, red!80] (sin \a, sin \a, \i/360) -- (sin \b, sin \b, \j/360);
		\else
		\draw [thick, red!80] (sin \a, sin \a, \i/360) -- (sin \b, sin \b, \j/360);
		\ifnum\c=1
		\draw [->,opacity=0.3] (0,0,\i/360) -- ++(sin \a, sin \a, 0);
		\fi
		\fi
	}
	\end{scope}
	
	\begin{scope}[shift={(0,0,6.125)}]
	
	\node [yslant=tan(\zangle), above=0.25cm, align=center,font=\footnotesize] at 
	(1,1,1.5){Unpolarized Light};
	
	\begin{scope}[xscale=1.5, yscale=1.5]
	\path [crystal!25, plate] 
	(-1,-1,0) -- (-1,1,0) -- (1,1,0) -- (1,-1, 0) -- cycle;
	\path [crystal!50, plate] 
	(-1,-1,0) -- (-1,-1,-0.0625) -- (-1,1,-0.0625) -- (-1,1, 0) -- 
	cycle;
	\path [crystal!75, plate] 
	(-1,1,0) -- (-1,1,-0.0625) -- (1,1,-0.0625) -- (1,1, 0) -- cycle;
	\node [yslant=tan(\xangle), text=crystal!50, below, font=\small] at 
	(-1,-1,0){45$^\circ$ Linear Polarizer};
	\end{scope}
	
	
	\draw [markerss] (-1.25,0.75) -- (-0.75,1.25);
	
	\draw [markerss] (-1.25,0.25) -- (-0.25,1.25);
	
	\draw [markerss] (-1.25,-0.25) -- (0.25,1.25);
	
	\draw [markerss] (-1.25,-0.75) -- (0.75,1.25);
	%up
	\draw [markerss] (-1.25,-1.25) -- (1.25,1.25);
	%down
	\draw [markerss] (-0.75,-1.25) -- (1.25,0.75);
	
	\draw [markerss] (-0.25,-1.25) -- (1.25,0.25);
	
	\draw [markerss] (0.25,-1.25) -- (1.25,-0.25);
	
	\draw [markerss] (0.75,-1.25) -- (1.25,-0.75);
	
	
	\foreach \k [evaluate={%
		\i=\k*5.625; \j=\i>0 ? \i-5.625 : 0; 
		\a=90-\i; 
		\b=90-\j; 
		\c=int(mod(\k,4)==0 && sin \a != 0); 
		\d=int(\k+1/4);}] in {0,...,192}{
		\ifodd\d
		\ifnum\c=1
		\draw [->,opacity=0.3] (0,0,\i/360) -- ++(sin \a, sin \a, 0);
		\fi
		\draw [thick,red!80] (sin \a, sin \a, \i/360) -- (sin \b, sin \b, \j/360);
		\else
		\draw [thick,red!80] (sin \a, sin \a, \i/360) -- (sin \b, sin \b, \j/360);
		\ifnum\c=1
		\draw [->,opacity=0.3] (0,0,\i/360) -- ++(sin \a, sin \a, 0);
		\fi
		\fi
	}
	
	\foreach \k [evaluate={%
		\i=\k*5.625; \j=\i>0 ? \i-5.625 : 0; 
		\a=90-\i; 
		\b=90-\j; 
		\c=int(mod(\k,4)==0 && cos \a != 0); 
		\d=int(\k+1/4);}] in {0,...,192}{
		\ifodd\d
		\ifnum\c=1
		\draw [->,opacity=0.3] (0,0,\i/360) -- ++(cos \a, 0, 0);
		\fi
		\draw [thick,teal] (cos \a, 0, \i/360) -- (cos \b, 0, \j/360);
		\else
		\draw [thick,teal] (cos \a, 0, \i/360) -- (cos \b, 0, \j/360);
		\ifnum\c=1
		\draw [->,opacity=0.3] (0,0,\i/360) -- ++(cos \a, 0, 0);
		\fi
		\fi
	}
	
	\foreach \k [evaluate={%
		\i=\k*5.625; \j=\i>0 ? \i-5.625 : 0; 
		\a=90-\i; 
		\b=90-\j; 
		\c=int(mod(\k,4)==0 && sin \a != 0); 
		\d=int(\k+1/4);}] in {0,...,192}{
		\ifodd\d
		\ifnum\c=1
		\draw [->,opacity=0.3] (0,0,\i/360) -- ++(0, sin \a, 0);
		\fi
		\draw [thick,orange] (0, sin \a, \i/360) -- (0, sin \b, \j/360);
		\else
		\draw [thick,orange] (0, sin \a, \i/360) -- (0, sin \b, \j/360);
		\ifnum\c=1
		\draw [->,opacity=0.3] (0,0,\i/360) -- ++(0, sin \a, 0);
		\fi
		\fi
	}
	
	\draw [ultra thick, ->] (0,0,3.5) -- (0,0,3);
	
	\end{scope}
	
	\end{tikzpicture}
